The ground-state potential and dipole moment of carbon monoxide: contributions from electronic correlation, relativistic effects, QED, adiabatic, and non-adiabatic corrections

The ground X1{\Sigma}+ state potential energy curve (PEC) and dipole moment curve (DMC) of CO molecule have been revisited within the framework of the relativistic coupled-cluster approach, which incorporates non-perturbative single, double, and triple cluster amplitudes (CCSDT) in conjunction with a finite-field methodology. The generalized relativistic pseudo-potential model was used for the effective introducing the relativity in all-electron correlation treatment and accounting the quantum-electrodynamics (QED) corrections within the model-QED-operator approach. The diagonal Born-Oppenheimer correction to PEC has been evaluated using the CCSD approach. The sensitivity of resulting PEC and DMC to variations in basis set parameters and regular intramolecular perturbations were considered as well. The present ab initio results are in a reasonable agreement with their most accurate semi-empirical counterparts.

==> table1.tex <==
\begin{table}
\begin{center}
\caption{\label{tab_basis}
Дипольный момент (в дебаях), рассчитанный методом CCSD, в зависимости от добавления дополнительных базисных функций. Третий столбец - изменение дипольного момента по отношению к значению, рассчитанному на предыдущем базисном наборе. Значения приведены для межъядерного расстояния 1.6 ангстрем c 10 скоррелированными электронами и учетом виртуальных орбиталей до 5 а.е.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{c c c}
% \toprule
              & d, D   &  $\Delta$d, D\\
\hline
  dyall.ae4z  & 0.5810 &         \\
  dyall.aae4z & 0.5830 &   0.0020\\
  +1s1p1d     & 0.5831 &   0.0002\\
  +1s1p1d1f   & 0.5839 &   0.0008\\
  +1s1p1d1f1g & 0.5839 &   0.0000\\
  +2s2p2d1f1g & 0.5836 &  -0.0003\\
  +2s2p2d2f1g & 0.5838 &   0.0002\\
  +2s2p2d2f2g & 0.5838 &   0.0000\\
% \bottomrule
\end{tabular}
\end{center}
\end{table}


==> table2.tex <==
\begin{table}
\begin{center}
\caption{\label{VIRT}
Изменение значения дипольного момента  (в дебаях), рассчитанного методами CCSD и CCSD(T),  при увеличении числа виртуальных орбиталей. Данные расчета для межъядерного расстояния 1.6 ангстрем.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{tabular}{cr@{}lr@{}lr@{}lr@{}lr@{}lr@{}lr@{}|}

\begin{tabular}{c c c}

\hline
 число виртуальных орбиталей  & $\Delta$d(CCSD), D & $\Delta$d(CCSD(T)), D \\ 
\hline
 64 (5 а.е.)                  &        &         \\
 131 (50 а.е.)                & 0.0647 &  0.0339 \\
 140 (100 а.е.)               & 0.0044 &  0.0031 \\
 174 (300 а.е.)               & 0.0002 &  0.0003 \\
 
\end{tabular}
\end{center}
\end{table}

